A large 'Active Magnetic Shield' for a high-precision experiment

We present a novel Active Magnetic Shield (AMS), designed and implemented for the n2EDM experiment at the Paul Scherrer Institute. The experiment will perform a high-sensitivity search for the electric dipole moment of the neutron. Magnetic-field stability and control is of key importance for n2EDM. A large, cubic, 5m side length, magnetically shielded room (MSR) provides a passive, quasi-static shielding-factor of about 10^5 for its inner sensitive volume. The AMS consists of a system of eight complex, feedback-controlled compensation coils constructed on an irregular grid spanned on a volume of less than 1000m^3 around the MSR. The AMS is designed to provide a stable and uniform magnetic-field environment around the MSR, while being reasonably compact. The system can compensate static and variable magnetic fields up to +-50muT (homogeneous components) and +-5muT (first-order gradients), suppressing them to a few muT in the sub-Hertz frequency range. The presented design concept and implementation of the AMS fulfills the requirements of the n2EDM experiment and can be useful for other applications, where magnetically silent environments are important and spatial constraints inhibit simpler geometrical solutions.

==> AMS-goals.tex <==
\begin{comment}

The n2EDM experiment is located in the vicinity of other research facilities using strong magnets producing fringe fields of several to several tens of \SI{}{\micro \tesla} at the n2EDM location.
Changes of these fields of the same order of magnitude occur frequently on timescales of minutes to hours. The AMS system aims to stabilize these magnetic fields, to which the Mu-metal is exposed. In turn this will decrease the change in magnetization of the outer most layer of the passive magnetic shield, increasing the overall stability of the magnetic environment. Furthermore, the AMS system will increase the shielding at sub-Hertz frequencies, with the goal to improve the overall shielding factor, the product of passive and active shield, by one order of magnitude.



\begin{figure}[ht]
\centering
\includegraphics[width=0.45\textwidth]{Images/AMS+MSR-names.png}
\caption{\label{fig:AMS_MSR} Frequency-dependent shielding-factors of the MSR (light green and colored curves for the spatial directions) measured by applying 2\,\SI{}{\micro \tesla} peak-to-peak field;  and expected shielding-factor improvements provided by the AMS system (dark green) for large disturbances of order several 10\,\SI{}{\micro \tesla} in the low-frequency range. Figure is adapted from~\cite{MSR2022}.}
\end{figure}

\end{comment}


%the shielding factor was measured with a sinusoidal \SI{2}{\micro \tesla} peak-to-peak signal.


==> Stability.tex <==
The stability of the magnetic field can be quantified with the Allan Standard Deviation (ASD)

Comparing Allan of uncompensated field to that of the measured magnetic field reveals if the noise level is
decreased by applying the AMS in dynamic mode. The ratio of both ASD shows the factor by which the stability was improved at a given integration time  for each specific measurement.


\begin{figure}[ht]
\centering
    \includegraphics[width=0.5\textwidth]{Images/QuSpin-ASD.png}
  \caption{The stability of the AMS compensation. The Allan deviation (ASD) of the magnetic-field is plotted as the function of integration time for the measurements inside the MSR with the AMS system in static (blue) and dynamic (yellow) modes.}
\label{fig:Qu-ASD}
\end{figure}
